Primordial helium abundance determination using sulphur as metallicity tracer

The primordial helium abundance $Y_P$ is calculated using sulphur as metallicity tracer in the classical methodology (with $Y_P$ as an extrapolation of $Y$ to zero metals). The calculated value, $Y_{P,\,S}=0.244\pm0.006$, is in good agreement with the estimate from the Planck experiment, as well as, determinations in the literature using oxygen as the metallicity tracer. The chemical analysis includes the sustraction of the nebular continuum and of the stellar continuum computed from simple stellar population synthesis grids. The $S^{+2}$ content is measured from the near infrared $\left[SIII\right]\lambda\lambda9069\AA,9532\AA$ lines, while an $ICF\left(S^{3+}\right)$ is proposed based on the $Ar^{3+}/Ar^{2+}$ fraction. Finally, we apply a multivariable linear regression using simultaneously oxygen, nitrogen and sulphur abundances for the same sample to determine the primordial helium abundance resulting in $Y_{P-O,\,N,\,S}=0.245\pm0.007$

==> tables/ionicAbundancesTable.tex <==
\begin{tabu}{lccccc}%
\hline%
HII Galaxy&$\nicefrac{He^{+}}{H^{+}}$&$\nicefrac{He^{2+}}{H^{+}}$&$12 + log\left(\nicefrac{O^{+}}{H^{+}}\right)$&$12 + log\left(\nicefrac{O^{2+}}{H^{+}}\right)$&$12 + log\left(\nicefrac{N^{+}}{H^{+}}\right)$\\%
\hline%
\href{http://dr12.sdss3.org/spectrumDetail?mjd=53725\&fiber=536\&plateid=2329}{FTDTR-1}&0.0977$\pm$0.0011&0.0012$\pm$0.0002&7.29$\pm$0.10&7.75$\pm$0.053&5.38$\pm$0.050\\%
\href{http://dr12.sdss3.org/spectrumDetail?mjd=51991\&fiber=312\&plateid=556}{IZw18}&0.0768$\pm$0.0028&0.00053$\pm$0.0&6.48$\pm$0.12&6.95$\pm$0.069&4.74$\pm$0.062\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=2211\&mjd=53786\&fiber=486}{MRK36-A1}&0.0795$\pm$0.0082&0.0018$\pm$0.0002&7.32$\pm$0.091&7.73$\pm$0.071&5.56$\pm$0.21\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=2211\&mjd=53786\&fiber=486}{MRK36-A2}&0.0801$\pm$0.0097&0.0012$\pm$0.0&7.68$\pm$0.051&7.68$\pm$0.038&5.67$\pm$0.33\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=1382\&mjd=53115\&fiber=175}{MRK475}&0.0883$\pm$0.0045&0.0017$\pm$0.0001&7.50$\pm$0.059&7.83$\pm$0.043&5.75$\pm$0.25\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=976\&mjd=52413\&fiber=600}{FTDTR-2}&0.0756$\pm$0.0033&0.0010$\pm$0.0002&-&7.88$\pm$0.069&5.53$\pm$0.067\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=1383\&mjd=53116\&fiber=110}{IZw70}&0.0943$\pm$0.0032&0.00058$\pm$0.0001&8.15$\pm$0.11&7.99$\pm$0.055&6.40$\pm$0.045\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=1388\&mjd=53119\&fiber=17}{MRK689}&0.0775$\pm$0.0068&-&8.35$\pm$0.095&8.19$\pm$0.049&6.31$\pm$0.041\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=2094\&mjd=53851\&fiber=487}{MRK67}&0.0910$\pm$0.012&0.00096$\pm$0.0&7.79$\pm$0.084&8.00$\pm$0.047&5.88$\pm$0.19\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=2233\&mjd=53845\&fiber=371}{FTDTR-3}&0.0847$\pm$0.0030&-&7.47$\pm$0.074&8.12$\pm$0.043&5.61$\pm$0.24\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=418\&mjd=51817\&fiber=302}{SHOC22}&0.0838$\pm$0.0018&0.0014$\pm$0.0001&7.97$\pm$0.13&7.97$\pm$0.069&6.24$\pm$0.055\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=861\&mjd=52318\&fiber=489}{FTDTR-4}&0.0878$\pm$0.0015&0.00075$\pm$0.0&7.87$\pm$0.11&7.85$\pm$0.028&6.04$\pm$0.049\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=550\&mjd=51959\&fiber=92}{SHOC220}&0.0989$\pm$0.0023&0.0018$\pm$0.0001&6.80$\pm$0.043&7.52$\pm$0.024&5.56$\pm$0.075\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=942\&mjd=52703\&fiber=612}{FTDTR-5}&0.0779$\pm$0.0042&-&-&8.06$\pm$0.11&-\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=456\&mjd=51910\&fiber=76}{FTDTR-6}&0.0869$\pm$0.0019&0.00088$\pm$0.0&7.80$\pm$0.090&8.00$\pm$0.045&5.84$\pm$0.16\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=1185\&mjd=52642\&fiber=123}{FTDTR-7}&0.0864$\pm$0.0013&0.00041$\pm$0.0&7.49$\pm$0.050&8.05$\pm$0.020&5.72$\pm$0.022\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=934\&mjd=52672\&fiber=369}{MRK627}&0.0845$\pm$0.0040&-&8.30$\pm$0.12&8.12$\pm$0.060&6.54$\pm$0.051\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=640\&mjd=52200\&fiber=270}{SHOC592}&0.0962$\pm$0.0080&-&7.74$\pm$0.061&8.18$\pm$0.043&6.59$\pm$0.037\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=376\&mjd=52143\&fiber=160}{PHL293B}&0.0766$\pm$0.0024&0.0017$\pm$0.0002&6.73$\pm$0.052&7.70$\pm$0.021&-\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=639\&mjd=52146\&fiber=242}{SHOC588}&0.0940$\pm$0.0084&0.00059$\pm$0.0&7.38$\pm$0.055&8.18$\pm$0.028&6.25$\pm$0.034\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=394\&mjd=51913\&fiber=472}{SHOC36}&0.102$\pm$0.010&0.0028$\pm$0.0007&6.75$\pm$0.046&7.69$\pm$0.038&5.57$\pm$0.051\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=358\&mjd=51818\&fiber=472}{SHOC575}&0.0977$\pm$0.0018&-&7.57$\pm$0.063&8.18$\pm$0.046&6.66$\pm$0.038\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=358\&mjd=51818\&fiber=504}{SHOC579}&0.0991$\pm$0.0049&0.00040$\pm$0.0&7.17$\pm$0.023&8.05$\pm$0.0057&6.35$\pm$0.014\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=942\&mjd=52703\&fiber=612}{FTDTR-8}&0.0750$\pm$0.0018&-&7.12$\pm$0.11&7.86$\pm$0.045&5.27$\pm$0.096\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=556\&mjd=51991\&fiber=224}{SHOC263}&0.0866$\pm$0.0056&-&8.19$\pm$0.11&8.04$\pm$0.057&6.63$\pm$0.053\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=501\&mjd=52235\&fiber=602}{FTDTR-9}&0.0890$\pm$0.0032&0.0016$\pm$0.0001&8.00$\pm$0.23&8.05$\pm$0.095&6.27$\pm$0.086\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=575\&mjd=52319\&fiber=521}{FTDTR-10}&0.0783$\pm$0.0026&0.0010$\pm$0.0002&7.22$\pm$0.13&7.79$\pm$0.071&5.79$\pm$0.21\\%
\hline%
HII Galaxy&$12 + log\left(\nicefrac{S^{+}}{H^{+}}\right)$&$12 + log\left(\nicefrac{S^{2+}}{H^{+}}\right)$&$ICF\left(S^{3+}\right)$&$12 + log\left(\nicefrac{Ar^{2+}}{H^{+}}\right)$&$12 + log\left(\nicefrac{Ar^{3+}}{H^{+}}\right)$\\%
\hline%
\href{http://dr12.sdss3.org/spectrumDetail?mjd=53725\&fiber=536\&plateid=2329}{FTDTR-1}&5.15$\pm$0.041&5.83$\pm$0.036&1.95$\pm$0.078&5.16$\pm$0.043&5.18$\pm$0.062\\%
\href{http://dr12.sdss3.org/spectrumDetail?mjd=51991\&fiber=312\&plateid=556}{IZw18}&4.62$\pm$0.050&5.08$\pm$0.048&1.37$\pm$0.046&4.55$\pm$0.056&4.16$\pm$0.090\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=2211\&mjd=53786\&fiber=486}{MRK36-A1}&5.31$\pm$0.038&5.97$\pm$0.035&1.26$\pm$0.045&5.40$\pm$0.037&4.78$\pm$0.080\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=2211\&mjd=53786\&fiber=486}{MRK36-A2}&5.43$\pm$0.024&6.16$\pm$0.021&1.22$\pm$0.018&5.53$\pm$0.023&4.79$\pm$0.037\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=1382\&mjd=53115\&fiber=175}{MRK475}&5.45$\pm$0.027&6.23$\pm$0.024&1.20$\pm$0.019&5.64$\pm$0.026&4.85$\pm$0.043\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=976\&mjd=52413\&fiber=600}{FTDTR-2}&5.28$\pm$0.054&5.99$\pm$0.046&1.50$\pm$0.082&5.38$\pm$0.058&5.07$\pm$0.10\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=1383\&mjd=53116\&fiber=110}{IZw70}&5.91$\pm$0.043&6.40$\pm$0.037&-&5.80$\pm$0.042&-\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=1388\&mjd=53119\&fiber=17}{MRK689}&5.93$\pm$0.039&6.56$\pm$0.033&-&5.84$\pm$0.038&-\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=2094\&mjd=53851\&fiber=487}{MRK67}&5.54$\pm$0.037&6.21$\pm$0.033&1.32$\pm$0.041&5.68$\pm$0.037&5.15$\pm$0.056\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=2233\&mjd=53845\&fiber=371}{FTDTR-3}&5.23$\pm$0.032&6.16$\pm$0.029&1.88$\pm$0.084&5.59$\pm$0.031&5.53$\pm$0.040\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=418\&mjd=51817\&fiber=302}{SHOC22}&5.77$\pm$0.053&6.42$\pm$0.045&1.28$\pm$0.054&5.74$\pm$0.051&5.14$\pm$0.087\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=861\&mjd=52318\&fiber=489}{FTDTR-4}&5.64$\pm$0.046&6.24$\pm$0.040&1.19$\pm$0.023&5.64$\pm$0.045&4.87$\pm$0.038\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=550\&mjd=51959\&fiber=92}{SHOC220}&4.73$\pm$0.024&5.58$\pm$0.017&1.79$\pm$0.062&5.02$\pm$0.030&4.93$\pm$0.028\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=942\&mjd=52703\&fiber=612}{FTDTR-5}&5.30$\pm$0.090&6.05$\pm$0.076&1.79$\pm$0.25&5.47$\pm$0.093&5.37$\pm$0.13\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=456\&mjd=51910\&fiber=76}{FTDTR-6}&5.48$\pm$0.037&6.36$\pm$0.033&1.26$\pm$0.032&5.72$\pm$0.036&5.06$\pm$0.050\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=1185\&mjd=52642\&fiber=123}{FTDTR-7}&5.27$\pm$0.020&6.09$\pm$0.017&1.69$\pm$0.040&5.50$\pm$0.019&5.34$\pm$0.020\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=934\&mjd=52672\&fiber=369}{MRK627}&5.99$\pm$0.049&6.55$\pm$0.041&-&5.89$\pm$0.049&-\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=640\&mjd=52200\&fiber=270}{SHOC592}&6.07$\pm$0.036&6.69$\pm$0.030&-&5.93$\pm$0.036&5.10$\pm$0.23\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=376\&mjd=52143\&fiber=160}{PHL293B}&5.12$\pm$0.031&5.95$\pm$0.031&1.57$\pm$0.054&5.35$\pm$0.031&5.09$\pm$0.036\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=639\&mjd=52146\&fiber=242}{SHOC588}&5.73$\pm$0.032&6.35$\pm$0.029&1.22$\pm$0.041&5.80$\pm$0.031&5.09$\pm$0.089\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=394\&mjd=51913\&fiber=472}{SHOC36}&5.22$\pm$0.033&5.91$\pm$0.031&1.77$\pm$0.16&5.25$\pm$0.049&5.16$\pm$0.099\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=358\&mjd=51818\&fiber=472}{SHOC575}&5.74$\pm$0.037&6.48$\pm$0.031&-&5.95$\pm$0.036&-\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=358\&mjd=51818\&fiber=504}{SHOC579}&5.54$\pm$0.014&6.36$\pm$0.015&1.31$\pm$0.016&5.76$\pm$0.013&5.19$\pm$0.020\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=942\&mjd=52703\&fiber=612}{FTDTR-8}&5.14$\pm$0.040&5.89$\pm$0.032&1.86$\pm$0.082&5.42$\pm$0.042&5.37$\pm$0.059\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=556\&mjd=51991\&fiber=224}{SHOC263}&6.00$\pm$0.046&6.60$\pm$0.049&-&5.87$\pm$0.044&-\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=501\&mjd=52235\&fiber=602}{FTDTR-9}&5.74$\pm$0.083&6.52$\pm$0.069&-&5.73$\pm$0.081&-\\%
\href{http://dr12.sdss3.org/spectrumDetail?plateid=575\&mjd=52319\&fiber=521}{FTDTR-10}&5.52$\pm$0.057&6.18$\pm$0.048&-&5.46$\pm$0.056&-\\%
\hline%
\end{tabu}
